Navigating the Python Type Jungle

Python's typing system has evolved pragmatically into a powerful but theoretically fragmented system, with scattered specifications. This paper proposes a formalization to address this fragmentation. The central contribution is a formal foundation that uses concepts from type theory to demonstrate that Python's type system can be elegantly described. This work aims to serve as a crucial first step toward the future development of type inference tools.

==> eptcsdata.tex <==
\providecommand{\firstpage}{79}
\providecommand{\publicationstatus}{Andrei Arusoaie, Hora\c{t}iu Cheval, Radu Iosif: FROM 2025\\
EPTCS 427, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.427.6}{10.4204/EPTCS.427.6}}

